2D Matryoshka Sentence Embeddings

Common approaches rely on fixed-length embedding vectors from language models as sentence embeddings for downstream tasks such as semantic textual similarity (STS). Such methods are limited in their flexibility due to unknown computational constraints and budgets across various applications. Matryoshka Representation Learning (MRL) \cite{aditya2022matryoshka} encodes information at finer granularities, i.e., with lower embedding dimensions, to adaptively accommodate \emph{ad hoc} tasks. Similar accuracy can be achieved with a smaller embedding size, leading to speedups in downstream tasks. Despite its improved efficiency, MRL still requires traversing all Transformer layers before obtaining the embedding, which remains the dominant factor in time and memory consumption. This prompts consideration of whether the fixed number of Transformer layers affects representation quality and whether using intermediate layers for sentence representation is feasible. In this paper, we introduce a novel sentence embedding model called \textit{Two-dimensional Matryoshka Sentence Embedding} (2DMSE)\footnote{Our code is available at \url{https://github.com/SeanLee97/AnglE/blob/main/README_2DMSE.md}.}. It supports elastic settings for both embedding sizes and Transformer layers, offering greater flexibility and efficiency than MRL. We conduct extensive experiments on STS tasks and downstream applications. The experimental results demonstrate the effectiveness of our proposed model in dynamically supporting different embedding sizes and Transformer layers, allowing it to be highly adaptable to various scenarios.

==> related_work.old.tex <==
This section is organized as follows: We first introduce complex embedding, then the unsupervised and the supervised text embedding approaches, and finally, we give a summary.

\input{table_related_work}


\paragraph{Complex Embedding} 
Complex embedding has been applied in various scenarios. In position embedding learning, \citet{su2021roformer} adopted the multiplication in complex space to implement rotary position embedding in the transformer architecture.
In knowledge graph learning, \citet{pmlr-v48-trouillon16} presented entity embedding in complex space for link prediction. \citet{sun2018rotate} further conducted multiplication between entity embeddings in complex space to implement rotation. To represent complex embedding, they use two different entity embeddings to represent the real part and the imaginary part of the complex vector, respectively. 
Different from them, we used the division in complex space to compute the angle difference between text embeddings to mitigate the negative effects of cosine saturation zones.

\paragraph{Unsupervised Text Embedding Approaches} 
% Early studies \citep{DBLP:conf/naacl/HillCK16,pagliardini-etal-2018-unsupervised} have demonstrated the efficacy of augmenting word2vec \citep{word2vec_mikolov_2013} with n-gram embeddings.
BERT-flow \citep{li-etal-2020-sentence} has introduced a flow-based approach that maps BERT embeddings to a standard Gaussian latent space. On the other hand, BERT-whitening \citep{su2021whitening} applies the whitening operation to BERT embeddings to enhance text embeddings.
Very recent research \citep{carlsson2020semantic, zhang-etal-2020-unsupervised, giorgi-etal-2021-declutr, simcse_gao_2021, consert_yan_2021, chuang-etal-2022-diffcse, promcse_jiang_2022, zhuo-etal-2023-whitenedcse} has focused on leveraging contrastive objectives for text embedding learning.

\paragraph{Supervised Text Embedding Approaches} Supervised text embeddings usually perform better than their unsupervised counterparts \citep{simcse_gao_2021}. Various studies have effectively utilized supervised datasets to enhance the learning of text embeddings. In particular, \citet{conneau-etal-2017-supervised} introduced a method that leverages supervised Natural Language Inference (NLI) tasks for this purpose. Building on a transformer backbone, USE \citep{cer-etal-2018-universal} incorporates the SNLI dataset to augment unsupervised training, resulting in improved performance. Furthermore, SBERT \citep{sbert-nils-2019} enhances text embedding by combining BERT with a siamese architecture.

Table \ref{table_related_work} lists the similarity measurements and learning algorithms of the widely used text embeddings. 
We can see that most existing works optimize the cosine similarity. 
However, none of the existing works considers the negative effect of cosine saturation zones. To address this issue, this paper proposes a novel angle-optimized text embedding model for text embedding learning.

==> table_downstream.tex <==
\begin{table*}[]
\setlength\tabcolsep{1.5pt}
\small
\centering
\begin{threeparttable}
\begin{tabular}{lcccccccc}
\toprule
Model $\downarrow$ & MR & CR & SUBJ & MPQA & SST2 & TREC & MRPC & Avg. \\

\midrule
\midrule
openai-ada-002 $\diamondsuit$  & $-$ & $-$ & $-$  & $-$  & $-$  & $-$   & $-$ & $90.10$ \\

GloVe $\dagger$ & $77.25$ & $78.30$ &  $91.17$ &  $87.85$ & $80.18$ &  $83.00$ & $72.87$ &  $81.52$ \\ 
Skip-thought $\ddagger$ & $76.50$ & $80.10$ & $93.60$ & $87.10$ &  $82.00$ & $92.20$ & $73.00$ & $83.50$ \\

Avg. BERT $\dagger$ & $78.66$ & $86.25$ & $94.37$ & $88.66$ &  $84.40$ & $92.80$ & $69.54$ & $84.94$ \\

BERT-CLS $\dagger$ & $78.68$ & $84.85$ & $94.21$ & $88.23$ & $84.13$ & $91.40$ & $71.13$ & $84.66$ \\

IS-BERT $\ddagger$ & $81.09$ & $87.18$ & $94.96$ & $88.75$ & $85.96$  & $88.64$ & $74.24$ &  $85.83$ \\

SimCSE-BERT$_{base}$ $\clubsuit$ & $81.18$ & $86.46$ & $94.45$ & $88.88$ & $85.50$ & $89.80$ & $74.43$ &  $85.81$ \\

SBERT$_{base} \star$ & $80.10$ & $86.25$ & $94.61$ & $88.78$ & $84.90$ & $89.00$ & $73.25$ &  $85.27$ \\
% DiffCSE-BERT$_{base}$ $\diamondsuit$ & $82.69$ & $87.23$ & $95.23$ & $89.28$ & $86.60$ & $90.40$ & $76.58$ & $86.86$ \\

% SimCSE-LLaMA $\star$ & $90.42$ & $92.89$ & $95.98$ & $91.37$ & $95.13$ & $95.40$ & $75.12$ & $91.06$ \\
\midrule
AoE-BERT$_{base}$ (ours) & $82.92_{ \pm 0.25}$ & $89.38_{ \pm 0.28}$ & $94.88_{ \pm 0.31}$ & $89.84_{ \pm 0.47}$ & $87.10_{ \pm 0.22}$ & $89.60_{ \pm 0.44}$ & $74.61_{ \pm 0.39}$ & $86.90$ \\

AoE-LLaMA$_{7B}$ (ours) & $90.66_{ \pm 0.29}$ & $93.48_{ \pm 0.31}$ & $96.27_{ \pm 0.38}$ & $91.78_{ \pm 0.47}$ & $94.67_{ \pm 0.30}$ & $95.80_{ \pm 0.58}$ & $74.32_{ \pm 0.41}$ & $91.00$ \\

AoE-LLaMA$_{13B}$ (ours) & $\mathbf{91.17}_{ \pm 0.32}$ & $\mathbf{93.54}_{ \pm 0.33}$ & $\mathbf{96.60}_{ \pm 0.42}$ & $\mathbf{91.98}_{ \pm 0.49}$ & $\mathbf{96.16}_{ \pm 0.25}$ & $\mathbf{96.80}_{ \pm 0.60}$ & $\mathbf{77.57}_{ \pm 0.42}$ & $\mathbf{91.97}$ \\

\bottomrule

\end{tabular}
\end{threeparttable}
\caption{
Results of text embeddings on the small-scale downstream tasks. 
The reported metrics is accuracy. 
$\diamondsuit$: results from \citep{ada_002};
$\dagger$: results from \citet{sbert-nils-2019}; $\ddagger$: results from \citet{zhang-etal-2020-unsupervised}; $\clubsuit$: results from \citet{simcse_gao_2021}; $\diamondsuit$: results from \citet{chuang-etal-2022-diffcse};
$\star$: results are our implementation using the official code. 
For our models, we report the average score over five runs. 
}
\label{table_downstream}
\end{table*}

==> table_github_statistic.tex <==
\begin{table}[]
    \small
    \centering
    \begin{tabular}{c|ccc}
    \toprule
    Split $\rightarrow$ & Train Set & Validation Set & Test Set \\
    \midrule
    \#Pos & $9457$ & $774$ & $807$ \\
    \#Neg & $9108$ & $773$ & $741$ \\
    \midrule
    Total & $18565$ & $1547$ & $1548$ \\
    \bottomrule
    \end{tabular}
    \caption{Data split and data size of the GIS dataset. \#Pos and \#Neg is the count of positive and negative pairs, respectively.}
    \label{table_github_statistics}
\end{table}

==> table_llm_sup.tex <==
\begin{table}[]
    \small
    \centering
    \begin{tabular}{lc}
        \toprule
        Model $\downarrow$ & Spearman's Correlation \\
        \midrule
        \midrule
        \multicolumn{2}{c}{\textit{Unsupervised Models}} \\
        \midrule
        SimCSE-BERT & $76.85$ \\
        ConSERT-BERT & $73.97$ \\
        DiffCSE-BERT & $80.59$ \\
        \midrule
        \midrule
        \multicolumn{2}{c}{\textit{LLM-supervised Models}} \\
        \midrule
        \textbf{AnglE-BERT} \\
        \ + ChatGPT annotator & $81.52$ \\
        \ + LLaMA2-7B annotator & $79.29$ \\
        \ + ChatGLM-6B annotator & $81.11$ \\
        \ + Ensemble LLM annotator & \cellcolor[HTML]{CCE5FF}$\mathbf{82.01}$ \\
        \bottomrule
    \end{tabular}
    \caption{Results of unsupervised and LLM-supervised models on the STS-B test set. 
    % For ChatGPT,  LLaMA, and ChatGLM, we use the gpt-turbo-3.5, 7B LLaMA2, and 6B ChatGLM, respectively.
    }
    \label{table_llm_sup}
\end{table}

==> table_main_nontransfer.tex <==
\begin{table}[ht]
\setlength\tabcolsep{4pt}
\small
\centering
\begin{threeparttable}
\begin{tabular}{lccc}
\toprule
    Model $\downarrow$ & STS-B & GIS & Avg. Spearman’s  \\
\midrule
\midrule

SimCSE & $76.27_{\pm 0.23}$ &  $60.38 _{\pm 0.18}$ & $68.33$ \\
SBERT & $84.67 _{\pm 0.35}$ &  $69.50 _{\pm 0.47}$ & $77.09$ \\
\midrule
AoE & $\mathbf{86.28}_{\pm 0.19}$ & $\mathbf{70.59}_{\pm 0.35}$ & $\mathbf{78.44}$ \\
\bottomrule
\end{tabular}
\end{threeparttable}
\caption{
Results of the in-domain STS tasks. 
All results of baselines are our implementation using their official code. BERT$_{base}$ is employed as the backbone for all models. Spearman's correlation ($\rho \times 100$) serves as the reported metric. We report the average Spearman's correlation score in five runs.
}
\label{table_indomain_sts}
\end{table}


==> table_related_work.tex <==
% move to appendix
\begin{table}[h]
\small
\centering
\begin{tabular}{lcc}
\toprule
\multicolumn{1}{c}{Model} & Use Cosine & Learning Algorithm                             \\ \midrule
\midrule
USE $\dagger$                     & \xmark                &  \multicolumn{1}{c}{Ensemble} \\ 
SBERT $\ddagger$                    & \cmark                 & \multicolumn{1}{c}{Regression} \\ 
SimCSE $\clubsuit$  & \cmark                  & Contrastive Learning                           \\ 
ConSERT $\diamondsuit$ & \cmark                  & Contrastive Learning                           \\ 
DiffCSE  $\heartsuit$    & \cmark                  & Contrastive Learning                           \\
PromptCSE   $\spadesuit$                & \cmark                  & Contrastive Learning                           \\
WhitenedCSE  $\blacklozenge$    & \cmark                  & Contrastive Learning                           \\ 
\bottomrule
\end{tabular}
\caption{The similarity measurements and learning algorithms of widely-used text embedding models. $\dagger$: \citet{cer-etal-2018-universal}. $\ddagger$: \citet{sbert-nils-2019}. $\clubsuit$: \citet{simcse_gao_2021}. $\diamondsuit$: \citet{consert_yan_2021}. $\heartsuit$: \citet{chuang-etal-2022-diffcse}. $\spadesuit$ is \citet{promcse_jiang_2022}. $\blacklozenge$: \citet{zhuo-etal-2023-whitenedcse}.
The majority of them used cosine to measure similarity.}
\label{table_related_work}
\end{table}

==> trash.tex <==
\subsection{Auxiliary Objective}
\label{sec::auxiliary}
The angle objective can be used alone for text embedding learning or combined with other auxiliary objectives to improve text embeddings further. 
% Here, we employ two widely adopted auxiliary objectives to improve AoE's robustness.
This multi-objective approach allows our proposed model to learn text embeddings comprehensively from multiple perspectives, enhancing the model's robustness.  Here, we employ the widely used supervised contrastive learning objective as the auxiliary objective $\mathcal{L}_{cl}$, as follows:
\begin{equation}
    \small
    \mathcal{L}_{cl} = - \sum_b \sum_i^m \mathrm{log} \left [ \frac{e^{\mathrm{cos}(\mathbf{X}_{b_i}, \mathbf{X}_{b_i}^+) / \tau}}{\sum_j^N e^{\mathrm{cos}(\mathbf{X}_{b_i}, \mathbf{X}_{b_j}^+) / \tau}} \right ],
\end{equation}
where $\tau$ is a temperature hyperparameter, $b$ stands for the $b$-th batch, $\mathbf{X}_{b_i}^+$ and $\mathbf{X}_{b_j}^+$ are the respective positive samples of $\mathbf{X}_{b_i}$ and $\mathbf{X}_{b_j}$, $m$ represents the number of positive pairs in $b$-th batch, $N$ is the batch size, and $\mathrm{cos}(\cdot)$ is the cosine similarity function.
Unlike existing contrastive learning models \citep{consert_yan_2021,promcse_jiang_2022,xu-etal-2023-distillcse} that generate positive samples through data augmentation, we use supervised positive samples. 
Additionally, we have observed the presence of identical sentences within a batch that are not explicitly labeled as positive samples. It may cause them to be treated as in-batch negatives. 
To address this issue, we propose an identical sentence pair (ISP) detection strategy. It enables AoE to assign these duplicate sentences as positive samples, effectively reducing potential noise in the data.

Finally, we combine the angle objective and the contrastive objective in the following manner to form the final objective function:
\begin{equation}
    \small
    \mathcal{L} = w_1 * \mathcal{L}_{angle} + w_2 * \mathcal{L}_{cl},
\end{equation}
where $w_1$ and $w_2$ are two hyperparameters to control the weights of different objectives. 
The negative effects of saturation zones can be mitigated using the angle objective.
% \textcolor{blue}{Although $\mathcal{L}_{cos}$ and $\mathcal{L}_{cl}$ optimize cosine with saturation zones, our angle optimization can mitigate their negative effects, as discussed in Section \ref{sec-ablation}.}



\paragraph{Discussion of LLM-supervised Learning.}

% \input{figure_llm_sup}
AoE, a supervised learning model, must be trained on labeled data. 
However, the limited availability of domain-supervised data poses a challenge in real-world applications. 
To overcome this problem, we propose LLM-supervised learning for STS. 
Specifically, we leverage LLMs as data annotators \citep{schick-schutze-2021-generating} to generate pseudo labels for domain-specific data, which are then utilized for training the STS model.
% Figure \ref{figure_llm_sup} outlines the procedures involved in LLM-supervised learning. 
To simulate domain application, we collect all ``sentence1'' texts from the STS-B train set and train the AoE model using LLM-supervised learning. 
The models are then tested on the STS-B test set.
% We compare the LLM-supervised AoE and widely used unsupervised contrastive learning models. 
Table \ref{table_llm_sup} shows the results. 
We can see that LLM-supervised AoE performs better than unsupervised contrastive baselines.
%, and the ensemble of LLMs achieves the best result. 
It suggests that LLM-supervised learning is effective for STS tasks and can alleviate the domain-supervised data scarcity problem.
% indicating that LLM-supervised learning can alleviate the domain-supervised data scarcity problem.


